Analytic Solutions of the Vector Burgers' Equation

The well-known analytical solution of Burgers' equation is extended to curvilinear coordinate systems in three-dimensions by a method which is much simpler and more suitable to practical applications than that previously used. The results obtained are applied to incompressible flow with cylindrical symmetry, and also to the decay of an initially linearly increasing wind.

==> orig/9410004.tex <==
%Paper: solv-int/9410004
%From: NERNEY@ssl.msfc.nasa.gov
%Date: Tue, 1 Nov 1994 10:05:51 -0600 (CST)

\leftskip=0pt \parskip=0pt \parindent=0pt
\tolerance 10000
% \font\eightrm=cmr8
% \font\tenrm=cmr10
\font\twelvebf=cmbx10 scaled 1200
\font\twelverm=cmr10 scaled 1200
\font\fourteenbf=cmbx10 scaled 1440
\nopagenumbers
\headline={\tenrm\hfil\folio}
\vskip .25in
\baselineskip=18pt
%\baselineskip = 2\baselineskip
%\voffset=2\baselineskip
\def\p#1 #2 {{{\partial #1}\over {\partial #2}}}
\def\ov#1 #2 {{{#1}\over {#2}}}
\vskip .5in
\centerline {\fourteenbf ANALYTIC SOLUTIONS OF THE VECTOR BURGERS' EQUATION}
\vskip .2in

\centerline {\twelverm Steven Nerney$^{1}$, Edward J. Schmahl$^{2}$
, and Z. E. Musielak$^{3}$}
$^1$ National Research Council Associate, NASA-Marshall Space Flight
Center, Alabama 35812.

$^2$ Astronomy Department, University of Maryland, College Park,
MD 20742.

$^3$ Department of Mechanical and Aerospace Engineering,
and Center for Space Plasmas and Aeronomic Research, University
of Alabama at Huntsville, Huntsville, Alabama 35899.\hfill
\bigskip
Accepted by the Quarterly of Applied Mathematics\hfill
\bigskip
September 3, 1993
\vskip .4in
%{\parindent =12pt \narrower\narrower\narrower
{\leftskip = 1in \rightskip =1in
{\bf Abstract.}
 The well-known analytical solution of Burgers' equation is extended
to curvilinear coordinate systems in three-dimensions by a method
which is much simpler and more suitable to practical applications
than that previously used [22]. The results obtained are applied
to incompressible flow with cylindrical symmetry, and also to the
decay of an initially linearly increasing wind. }
\medskip

\vskip .4in
%\baselineskip = 2\baselineskip
{\bf 1. Introduction}
\vskip .1in
Burgers' equation is a well-known example of a
non-linear partial differential equation whose solution can be
constructed
from a linear partial differential equation. It is, to the best
of our knowledge, the only such example. Much of the interest
in this equation arises because it is a very simple form of the
Navier-Stokes equation in the one-dimensional, cartesian,
time-dependent,
compressible, viscous limit [17]. An early study derived two
steady-state solutions [1],
and then the equation was used in studying the decay of free
turbulence [4,5]. The importance of the equation is due to the
non-linear term, $u\p  u x $, which allows the calculation of the
modification of the velocity due to the exchange of momentum
between a variety of different length scales. Burger's equation
is the simplest type that shows the complicated interplay between
the non-linear steepening and diffusion of a wave. \par
\medskip
The first full solution of the one-dimensional Burgers' equation was
found independently by both Cole [7] and Hopf [12]. Recently, the
solution has been extended to n-dimensions by using group action
on coset bundles [22]. The basic idea of this approach is to determine
coset spaces for a chosen group and for a chain of closed subgroups,
and then to construct a bundle out of these spaces. Next, the action
of the group on the bundle is prescribed and a class of tensor-valued
functions called invariants on the coset bundle is introduced. Because
these group invariants take the form of differential equations,
the method has been used to obtain a tensor version of the
n-dimensional Burgers' equation and to show that its solutions can
be constructed from a linear tensor diffusion equation. It has
also been demonstrated that the procedure gives a nonlinear tensor
equation for a generalized Burgers' equation with a higher than second
order derivative. In this
paper, we examine extensions of the basic class of solutions of the
vector Burgers' equation, which we discovered before we became aware of
 the work of Wolf et al., to more than one dimension and to curvilinear
coordinate systems. The main advantage of our approach is that it
is extremely simple from a mathematical point of view and that the
results we obtain have the potential to be used in a number of
applications
(see Section III for two simple applications). It must be added,
however, that the solutions obtained in this paper represent a
subclass of more general solutions to the tensor Burgers' equation
discussed by Wolf et al. [22].
\medskip
In what follows, we recapitulate part of the historical derivation
presented first by Cole [7] and Hopf [12]. This derivation is central
to our results in Sections II and III.
\medskip
The equation to be solved is
$$ \p u t + u\p u x = \nu {{\partial ^2u }\over
{\partial x^2}} ,\eqno (1)$$
where $\nu $ is a physical constant (viscosity).
A successful transformation uses
$$ u = \p {\phi } x ,\quad   \phi = \phi(x,t).\eqno (2)$$
Substituting into eq. (1) and integrating term-by-term with respect to
x
$$ \p {\phi } t  + {{1}\over {2}} \left (\p {\phi } x \right )^2 = \nu
\p {^2\phi } {x^2} ,\eqno (3)$$

where the function of integration is omitted. Because eq.
(3) is invariant under the transformation
$$ x\rightarrow ax ,\eqno (4a)$$
$$ t\rightarrow a^2t{ },\eqno (4b)$$
(a=constant), as is the diffusion equation,
this suggests that there exists a solution of the form
$$ \phi (x,t) = \phi (\theta (x,t)),\eqno (5)$$
where $\theta $ is a solution of the diffusion equation
$$ \p {\theta } t  = \nu {{\partial ^2\theta  }\over
{\partial x^2}}.\eqno (6)$$
Substitution into eq. (3) while subtracting eq. (6) gives
$$ \left (\ov {d\phi } {d\theta } \right )^2 = 2\nu  \ov {d^2\phi }
{d\theta ^2} ,\eqno (7a)$$
whose solution is
$$ \phi (\theta ) = -2\nu { }\ln { }(\theta - c_1) + c_2,\eqno (7b)$$
so that by choosing $c_1$=0
$$ u(x,t) = {{-2\nu }\over {\theta }}\p {\theta } x .\eqno (8)$$
Quite an interesting literature has developed around applications
of the solutions in pure mathematics [20],
magnetohydrodynamics [9], astrophysics [14,16], and cosmology
[10,15].
Lighthill [18] extended the basic transformation to the case
where the
x coordinate is measured in the frame of reference moving in the same
direction as the wave at the undisturbed speed of sound.
A valuable book on Burgers' equation and related topics was
recently published but is, unfortunately, already out of print [11].
\medskip
In the following, we formally present the derivation of
the solutions to the vector Burgers' equation by using a
generalized Cole-Hopf transformation.
\vskip .1in
{\bf 2. The Vector Extension of Burgers' Equation}
\vskip .1in
We begin with the vector equivalent of Burgers' equation
$$ \p  {\vec u} t  + \vec u\cdot \nabla \vec u = \nu \nabla ^2\vec u.
\eqno (9)$$
In order to evaluate the vector Laplacian we must use
$$ \nabla ^2\vec u = \nabla (\nabla \cdot \vec u) - \nabla \times
\nabla \times \vec u,\eqno (10a)$$
and for the inertial term
$$ \vec u\cdot \nabla \vec u = \nabla \ov  {u^2} 2  - \vec u\times
\nabla \times \vec u.\eqno (10b)$$
Then eq. (9) greatly simplifies as long as
$$\vec u\times \nabla \times \vec u = \nu \nabla \times \nabla \times
\vec u.\eqno (10c)$$
This appears to be an equation that represents quite general flows,
but the only solutions are irrotational. This can be seen by taking
the divergence of both sides of eq. (10c) and using
$$\nabla \cdot (\vec A\times \vec B) = \vec B\cdot \nabla \times
\vec A - \vec A\cdot \nabla \times \vec B.\eqno (10d)$$
In what follows we will assume that the flow field is irrotational
as this is necessary to simplify eq. (9) and to derive the
extension of the Cole-Hopf transformation. The assumption is
satisfied trivially for the one-dimensional Cartesian problem.
$$ \nabla \times \vec u = 0,\eqno (11a)$$
so that
$$ \vec u = \nabla \phi .\eqno (11b)$$
Eq. (11b) is the extension of eq. (2) to three dimensions and,
together with eqs. (10) allows
the simplification of eq. (9) to
$$ \nabla \left [\p {\phi } t  + {{(\nabla \phi )^2}\over {2}} -
\nu \nabla ^2\phi \right ] = 0.\eqno (12)$$
The meaning of eq. (12) is that the quantity enclosed by brackets must
be a function of time, only, because its gradient is zero in all space
so that
$$ \p {\phi } t  + {{(\nabla \phi )^2}\over {2}} -
\nu \nabla ^2\phi  = E(t).\eqno (13)$$
The form of the unknown function E(t) is irrelevant for our discussion
as it cannot affect the velocity. We simply define a new potential
$$ \phi _1 = \phi -\int E(t)dt,$$ where the gradients of $\phi $ and
$\phi _1$ are identical.
\medskip
Before introducing the Cole-Hopf assumption, it is useful to state the
following vector identity:
$$ \nabla \alpha  = \p  {\alpha } {\theta } \nabla \theta ,\eqno (14a)$$
which is true for any orthogonal, curvilinear coordinate system.
Taking the divergence of both sides with $\alpha =\phi $ and using eq.
(14a) again with $\alpha =\p {\phi } {\theta } $ yields
$$ \nabla ^2\phi  = \p {^2\phi } {\theta ^2} \thinspace
(\nabla \theta )^2 +
\p {\phi } {\theta } \thinspace \nabla ^2 \theta .\eqno (14b)$$
We will also need the diffusion equation
$$ \p {\theta } t  = \nu \nabla ^2\theta .\eqno (15)$$
Now we apply eqs. (5), (14b), and (15) to eq. (13) to generate eq.
(7a), again, so that
$$ \vec u = -\ov {2\nu } {\theta } \thinspace \nabla \theta
.\eqno (16)$$
This clearly shows that the Cole-Hopf transformation goes through
for quite general coordinate systems.
Cole [7] originally discussed the vector solution
for the case of cartesian coordinates and he indicated
that it applied to some
special solutions in higher dimensions.
\medskip
The usefullness of eq. (16) can be shown by exploiting the simple
symmetry of the following example.
\vskip .1in
\centerline {\bf 3. Cylindrical Symmetry}
\vskip .1in
Using only a radial velocity,
Burgers' equation in cylindrical coordinates with axisymmetry
may be written as
$$ \p  u t  + u\p  u r  = \nu \left [\ov  1 r \p  { } r \left (
r\p  u r \right ) - \ov  u {r^2} \right ]\eqno (17)$$
Equation (17) can be written as
$$ \p  u t  + u\p  u r  = \nu  \p  { } r \left (\ov  1 r \p  { } r
(ru)\right )\eqno (18)$$
Equation (18) and the related integrals of (18) are what led us to believe
that the Cole-Hopf transformation was quite general in nature.
The particular form of (16) is
$$ u = \ov  {-2\nu } {\theta } \p  {\theta } r \eqno (19)$$
where the diffusion equation is
$$ \p  {\theta } t  = \ov  {\nu } r \p  { } r \left (r\p
{\theta } r \right )\eqno (20)$$
A simple example of the use of this method is to use the initial-value
solution of the diffusion equation (a Dirac delta at t=r=0)
$$ \theta  = \ov  1 {2\nu t} e^{-{{r^2}\over {4\nu t}}} \eqno (21)$$
Then the solution of (17) is found from (19)
$$ u = {{r}\over {t}}\eqno (22)$$

This is the cylindrical version of Burgers' cartesian solution [4],
$u=x/t$, which is the inviscid solution of (1),
(solution 2.1, figure 5 in Benton [3]). Because (22) satisfies (17)
in the limit that $\nu \rightarrow 0$ (which is also the case of zero
acceleration for fluid particles), this solution is the inviscid
limit of the solution of Burgers' equation in cylindrical coordinates.
 Some solutions of (17), such as example B below, approach the
sawtooth limit as $t\rightarrow \infty $; but this is not
surprising as it has been
noted [2,13] that  the
sawtooth shape of dissipation layers is of fundamental importance
in Burgers' representation of turbulence.
\medskip
It is extremely useful to derive solutions of the diffusion equation
which are based on physical boundary conditions on the velocity field.
To this end,
equation (19) may be formally integrated to
$$ \theta (r,t) = k(t)\thinspace \exp \left (-{{1}\over
{2\nu }}\int _0^r u(w,t)\thinspace dw\right )\eqno (23)$$
where
$$ k(t) = \theta (0,t)\eqno (24)$$
The velocity is to be initially specified over a given range so
that the initial value of $\theta $ is given by
$$ \theta (r,0) = \theta _0(r) = k_0\thinspace \exp \left (-{{1}\over
{2\nu }}\int  u_0(w)\thinspace dw\right )\eqno (25)$$
for  $r_0\le r\le R$.
\medskip
The general solution of the diffusion equation, (20),
with azimuthal symmetry, is [19]
$$ \theta (r,t) = \int _0^\infty {\int _0^\infty  \theta _0(r^\prime )
J_0(kr^\prime )J_0(kr)e^ {-\nu k^2t}k\thinspace r^\prime dk}\thinspace
dr^\prime \eqno (26)$$
The integral over k can be done once and for all as it is
a special case of Weber's second exponential
integral as discussed in Watson [21].
$$ \int _0^\infty \exp (-\nu tk^2)J_0(kr)J_0(kr^\prime)k\thinspace
dk = {{1}\over {2\nu t}}\exp \left (-{{r^2+r^{\prime ^2}}\over {4\nu t}
}\right )I_0\left ({{r\thinspace r^\prime }\over {2\nu t}}\right )
\eqno (27)$$
where the modified Bessel function of order zero may be written as
$$ I_0(\alpha r^\prime) = J_0(i\alpha r^\prime )\eqno (28)$$
which is a real function.
Equation (26) may now be written as
$$ \theta (r,t) = \ov  1 {2\nu t} \exp {\left (-\ov  {r^2} {4\nu t}
\right )}
\int _0^{\infty }\theta _0(r^{\prime })\exp {\left
(- \ov  {r^{\prime 2}} {4\nu t} \right )}\thinspace J_0\left (\ov
{ir^{\prime }r} {2\nu t} \right )r^{\prime }dr^{\prime } \eqno (29)$$
\vskip .1in
\centerline {\bf 4. Two Simple Examples}
\vskip .1in
We choose to work two relatively simple examples so as not to obscure
the simple nature of the transform. It is surprisingly easy to pose
apparently straight-forward problems that cannot be readily carried
to completion because of extremely difficult quadratures. We will treat
 the more difficult case of the decay of an initially
constant velocity wind in a future paper.
\medskip
The reader may have noticed by now that Burger's equation does not
specify the density distribution except in a few limits
besides the trivial one of constant density.
\medskip
{\bf A. Incompressible Flow}
\smallskip
The first case is that of incompressible flow where we take a source
of water emanating from the origin of coordinates
and spreading out in a circularly symmetric pattern.
The initial flow is assumed to
exist from very close to r=0 out to R, which is assumed to be larger
than any other length scales in the problem. We then take the limit
as $R\rightarrow \infty $, in the same spirit as other studies of this
initial-value problem on infinite intervals [2].
The speed must decrease as
$r^{-1}$ to conserve mass in an initially steady flow.
In sum,
$$ u(r,0) = u_0\ov  {r_0} r \eqno (30)$$

$$ r_0\le r\le R $$

so that (25) integrates to
$$ \theta _0 = k_0\left (\ov  {r_0} r \right )^a\eqno (31)$$
where
$$ a = \ov  {u_0r_0} {2\nu } \eqno (32)$$
Clearly, $u_0$ may be large at the small value $r_0$ in such a way
that the product $u_0r_0$ is well-defined.
Equation (29) can now be integrated using Hankel's generalization
of (27) as discussed in Watson [21], so that
$$ \theta = k_0r_0^a \thinspace \Gamma \left (1-\ov  a 2
\right )\thinspace
(4\nu t)^{-a/2}\sum _{n=0}^\infty \ov  {\left (\ov  a 2 \right )_n}
{(n!)^2} \left (-\ov  {r^2} {4\nu t} \right )^n\eqno (33)$$
where $\left (\ov  a 2 \right )_n$ is Pochhammer notation,
$$\left (\ov  a 2 \right )_n =  \ov  a 2 \left (\ov  a 2 +1\right )
\left (\ov  a 2 +2\right )....
\left (\ov  a 2 +n-1\right )\eqno (34)$$
and
$$ \left (\ov  a 2 \right )_0 = 1 \eqno (35)$$
The full non-linear solution can now be derived from (19)
and expressed in terms of the confluent hypergeometric
function as
$$ u(r,t) = \ov  a 2 \ov  r t \ov  {M(a/2+1,2,-r^2/4\nu t)} {M(a/2,
1,-r^2/4\nu t)} \eqno (36a)$$
or more clearly as
$$ u(r,t) = \ov  r t \thinspace \ov  {\sum_{n=1}^\infty
(\ov  a 2 )_n\thinspace \ov
n {(n!)^2} \left (-\ov  {r^2} {4\nu t} \right )^{n-1}} {\sum_{n=0}
^\infty \ov  1 {(n!)^2} (\ov  a 2 )_n\left (-\ov  {r^2} {4\nu t}
\right )^n} \eqno (36b)$$

We see that the solution can be written as the product of the inviscid
solution times an infinite sum of powers of the similarity variable
$\ov  {r^2} {4\nu t} $. We note the non-linear effect on higher powers
of the similarity variable through the occurrence of the factor n in
the numerator. The transient non-linearly steepens but diffusion
dominates;
note that the transient is not by itself a solution of Burgers'
equation as we do not have the superposition theorem of linear
theory.
\medskip
Figure 1 was created by non-dimensionalizing equation (17) in the
usual fashion, i.e., $r\rightarrow r/L, t\rightarrow \nu t/l^2,
u\rightarrow u/U$. Choosing $U=u_0$ and $L=r_0$, then a is .5.
This ratio of series is initially divergent and required 100 terms
in double precision on a Sun SPARCstation.
The solutions are presented as isochrones, showing the evolution
of the non-linear solution towards a steady-state. The boundary where
the wind was turned off moves outward while diffusion smooths out
the discontinuity. The wind initially
drops off as 1/r so that the peak in the profile approaches the
starting radius for the source as $t\rightarrow 0$. All curves approach
 the steady-state envelope of 1/r while diffusion flattens the leading
edge. Asymptotically the velocity is zero everywhere.
\medskip
{\bf B. The Decay of An Initially Linearly Increasing Wind}
\medskip
Example two is a wind emanating from the origin, again,
but now the velocity linearly increases in magnitude out to
some radius, $r_0$, chosen to be larger than any other length scale
in the problem. We had in mind the initial theoretical treatments
of radiatively-driven winds [6] from early-type stars, but our
description is too simple to be applied to this problem. This is
because of our assumption of cylindrical rather than spherical
symmetry, and also because other effects are now known to be
important in these winds [8].
\medskip
The driving force is imagined to turn-off
at t=0, and then we calculate the decay of the flow.
In sum
$$ u(r,0) = u_0\ov  r {r_0} = \ov r {t_0} \eqno (37a)$$
$$ 0\le r\le r_0  ;\quad t=0$$
where
$$ t_0 = \ov  {r_0} {u_0} \eqno (37b)$$
is half the time for the wind to flow from the source to the
initial outer boundary. Both $r_0,u_0$ are large, but $t_0$ is not
necessarily big.
Then
$$ \theta _0 = k_0\thinspace e^{-br^2} \eqno (38)$$
$$ b = \ov  {u_0} {4\nu r_0} \eqno (39)$$
Proceeding as before
$$ \theta  = \ov  {k_0} {1+\ov  t {t_0} } \exp \left [-\ov  {r^2}
{4\nu t} \thinspace \ov  1 {1+\ov  {t_0} t } \right ]\eqno (40)$$
$$ u(r,t) = \ov  r {t+t_0} \eqno (41)$$
We note that the solution approaches the Burgers' sawtooth
shape as $t\rightarrow \infty $.
\vskip .1in
\centerline {\bf 5. Conclusions}
\vskip .1in
We have given a relatively simple proof that Burgers' equation can
be solved for curvilinear coordinate systems in three dimensions by
assuming irrotational flow and using equation (16) with $\theta $
derived from solutions of the diffusion equation.
We solved two examples in cylindrical coordinates
with circular symmetry to show how to implement the generalized
solution.
Our goal has been to extend the tools of workers who model the
complicated interplay between non-linear steepening
and viscous diffusion in waves.
\vskip .1in
{\bf Acknowledgments.}
\vskip .1in
ZEM acknowledges partial support of this work by the NSF under grant
no. ATM-9119580. EJS acknowledges partial support of this work
under grant no. NAG 2001 from NASA-Goddard Space Flight Center.
\vskip .1in
\centerline {References}
\vskip .1in

[1] H. Bateman, {\it Some recent researches on the motion of fluids},
Mon. Weather Rev. {\bf 43}, 163, (1915).

[2] E. R. Benton, {\it Solutions illustrating the decay of dissipation
layers in Burgers' nonlinear diffusion equation}, Phys. Fluids,
{\bf 10}, 2113, (1967).

[3] E.R. Benton, {\it A table of solutions of the one-dimensional
Burgers equation}, Q. Appl. Math., {\bf 30}, 195, (1972).

[4] J. M. Burgers, {\it Application of a model system to illustrate
some
points of the statistical theory of free turbulence},
Proc. Roy. Neth. Acad. Sci. Amsterdam {\bf 43}, 1, (1940).

[5] ----, {\it The Non-Linear Diffusion Equation}, D. Reidel Pub. Co.,
Dordrecht-Holland, 1974.

[6] J.I. Castor, D.C. Abbott, and R.I. Klein, {\it Radiatively-driven
winds in Of stars}, Astrophys. J.,
{\bf 195}, 157, (1975).

[7]  J. D. Cole, {\it A quasi-linear parabolic equation in
aerodynamics},
Quart. Appl. Math., {\bf 9}, 225, (1951).

[8] D.B. Friend, and D.C. Abbott, {\it The theory of radiatively-driven
 stellar winds. III. Wind models with finite disk correction and
rotation}, Astrophys. J., {\bf 311}, 701, (1986).

[9] Z. A. Gol'berg, {\it Finite amplitude waves in
magnetohydrodynamics},
 JETP, {\bf 15}, 179, (1962).

[10] S. N. Gurbatov, A. I. Saichev, and S. F. Shandarin,
{\it The large-scale structure of the universe in the frame of the
model of non-linear diffusion},
Mon. Not. R. Astr. Soc., {\bf 236}, 385, (1989).

[11] S.N. Gurbatov, A.N. Malakhov, and A.I.Saichev, {\it Nonlinear
random waves and turbulence in nondispersive media: waves, rays, and
particles}, (Manchester University Press, distributed by St.
Martin's Press, New York, 1991).

[12] E. Hopf, {\it The partial differential equation $u_t+uu_x=\mu
u_{xx}$
}, Comm. Pure and Appl. Math., {\bf 3}, 201, (1950).

[13] D.T. Jeng, R. Foerster, S. Haaland, and W.C. Meecham,
{\it Statistical initial-value problem for Burgers' model equation
of turbulence}, Phys. Fluids, {\bf 7}, 2114, (1966).

[14] J. I. Katz and M. L. Green, {\it A Burgers model of
interstellar dynamics}, Astron. Astrophys.,
{\bf 161}, (1986).

[15] L. A. Kofman and S. F. Shandarin, {\it Theory of adhesion for the
large-scale structure of the universe}, Nature, {\bf 334}
, 129, (1988).

[16] L.A. Kofman and A. C. Raga, {\it Modeling structures of knots in
jet flows with the Burgers equation}, Astrophys. J., {\bf 390}
, 359, (1992).

[17] P. Lagerstrom, J. D. Cole, and L. Trilling, {\it Problems in the
Theory of
Viscous Compressible Fluids}, monograph, California Institute of
Technology, (1949).

[18] M. J. Lighthill, {\it Viscosity effects in sound waves of finite
amplitude}, {\it Surveys in Mechanics}, ed.
Batchelor and Davies,
Cambridge Univ. Press, Cambridge, 1956.

[19] H. Margenau and G.M. Murphy, {\it The Mathematics of
Physics and Chemistry},
Von Nostrand Co., London, 1956.

[20] B. Van Der Pol, {\it On a non-linear partial differential
equation
satisfied by the logarithm of the Jacobian theta-functions, with
arithmetical application}, Proc. Acad. Sci. Amsterdam,
{\bf A13}, 261, (1951).

[21] G.N. Watson, {\it A Treatise on the Theory of Bessel Functions},
 second ed., (Cambridge Univ. Press, Cambridge, 1962, pg. 393-396).

[22] K. B. Wolf, L. Hlavaty, and S. Steinberg, {\it Non-linear
differential
equations as invariants under group action on coset bundles: Burgers
and Korteweg-de Vries equation families}, J. Math. Anal. and Applic.,
{\bf 114}, 340, (1986).

\eject
\centerline {\bf Figure Caption}
The non-linear evolution of a wind with an initial spatial dependence
of 1/r. The isochrones show the decay of the wind, and, especially,
the diffusion at the leading edge where the wind was turned off as
this discontinuity propagates outward.
\bye
%!PS-Adobe-3.0
%%BoundingBox: 54 54 558 738
%%Title: Graphics produced by IDL
%%For: schmahl@hesperia, /home/ed/Nerney
%%Creator: IDL Version 3.0.0 (sunos sparc)
%%CreationDate: Mon Apr 12 17:13:44 1993
%%DocumentData: Clean7bit
%%LanguageLevel: 1
%%PageOrder: Ascend
%%Pages: (atend)
%%DocumentNeededResources: (atend)
%%EndComments
%%BeginProlog
%+ prolog.ps -- Prolog for IDL generated PostScript files
%+ Copyright (c) 1988-1992 Research Systems, Inc. All Rights Reserved.
%v 2
save /$IDL_DICT 40 dict def $IDL_DICT begin /bdef { bind def } bind def /C
{currentpoint newpath moveto} bdef /CP {currentpoint} bdef /D {currentpoint
stroke moveto} bdef /F {closepath fill} bdef /K { setgray } bdef /M {moveto}
bdef /N {rmoveto} bdef /P {lineto} bdef /R {rlineto} bdef /S {gsave show
grestore} bdef /X {currentpoint pop} bdef /Z {gsave currentpoint lineto 20
setlinewidth 1 setlinecap stroke grestore} bdef /L0 {[] 0 setdash} bdef /L1
{[40 100] 0 setdash} bdef /L2 {[200 200] 0 setdash} bdef /L3 {[200 100 50
100] 0 setdash} bdef /L4 {[300 100 50 100 50 100 50 100] 0 setdash} bdef /L5
{[400 200] 0 setdash} bdef end 2.5 setmiterlimit
%%EndProlog
%%Page: 0 1
%%PageResources: (atend)
%%PageOrientation: Landscape
%%PageBoundingBox: 54 54 558 738
%%BeginPageSetup
save $IDL_DICT begin 54 738 translate 0.0283465 dup scale 270 rotate
%%IncludeResource: font Helvetica
/Helvetica findfont 423.333 scalefont setfont
%%EndPageSetup
20 setlinewidth L0 0.000 K 5484 17445 M 0 -552 R D 5958 17182 M -27 52 R
-79 27 R -78 0 R -79 -27 R -27 -52 R 27 -53 R 52 -26 R 132 -26 R 52 -27 R
27 -52 R 0 -27 R -27 -52 R -79 -26 R -78 0 R -79 26 R -27 52 R D
6247 17261 M -53 -27 R -52 -52 R -27 -79 R 0 -53 R 27 -79 R 52 -52 R
53 -26 R 79 0 R 52 26 R 53 52 R 26 79 R 0 53 R -26 79 R -53 52 R -52 27 R
-79 0 R D 6930 17182 M -52 52 R -53 27 R -79 0 R -52 -27 R -53 -52 R
-26 -79 R 0 -53 R 26 -79 R 53 -52 R 52 -26 R 79 0 R 53 26 R 52 52 R D
7114 17445 M 0 -552 R D 7114 17155 M 79 79 R 53 27 R 79 0 R 52 -27 R
26 -79 R 0 -262 R D 7614 17261 M 0 -368 R D 7614 17103 M 26 79 R 53 52 R
52 27 R 79 0 R D 8061 17261 M -53 -27 R -52 -52 R -27 -79 R 0 -53 R 27 -79 R
52 -52 R 53 -26 R 79 0 R 52 26 R 53 52 R 26 79 R 0 53 R -26 79 R -53 52 R
-52 27 R -79 0 R D 8455 17261 M 0 -368 R D 8455 17155 M 79 79 R 53 27 R
78 0 R 53 -27 R 26 -79 R 0 -262 R D 8928 17103 M 316 0 R 0 52 R -27 53 R
-26 26 R -52 27 R -79 0 R -53 -27 R -52 -52 R -27 -79 R 0 -53 R 27 -79 R
52 -52 R 53 -26 R 79 0 R 52 26 R 53 52 R D 9691 17182 M -27 52 R -78 27 R
-79 0 R -79 -27 R -27 -52 R 27 -53 R 52 -26 R 132 -26 R 52 -27 R 27 -52 R
0 -27 R -27 -52 R -78 -26 R -79 0 R -79 26 R -27 52 R D 10400 17261 M
-52 -27 R -53 -52 R -26 -79 R 0 -53 R 26 -79 R 53 -52 R 52 -26 R 79 0 R
53 26 R 53 52 R 26 79 R 0 53 R -26 79 R -53 52 R -53 27 R -79 0 R D
10953 17445 M -53 0 R -53 -27 R -26 -79 R 0 -446 R D 10742 17261 M 184 0 R D
11531 17445 M 0 -552 R D 11531 17445 M 368 -552 R 0 552 R D 12214 17261 M
-52 -27 R -53 -52 R -26 -79 R 0 -53 R 26 -79 R 53 -52 R 52 -26 R 79 0 R
53 26 R 52 52 R 27 79 R 0 53 R -27 79 R -52 52 R -53 27 R -79 0 R D
12609 17261 M 0 -368 R D 12609 17155 M 79 79 R 52 27 R 79 0 R 53 -27 R
26 -79 R 0 -262 R D 13108 17445 M 0 -552 R D 13292 17445 M 27 -27 R 26 27 R
-26 26 R -27 -26 R D 13319 17261 M 0 -368 R D 13529 17261 M 0 -368 R D
13529 17155 M 79 79 R 52 27 R 79 0 R 53 -27 R 26 -79 R 0 -262 R D
14002 17103 M 316 0 R 0 52 R -27 53 R -26 26 R -53 27 R -78 0 R -53 -27 R
-53 -52 R -26 -79 R 0 -53 R 26 -79 R 53 -52 R 53 -26 R 78 0 R 53 26 R
53 52 R D 14791 17261 M 0 -368 R D 14791 17182 M -53 52 R -52 27 R -79 0 R
-53 -27 R -52 -52 R -27 -79 R 0 -53 R 27 -79 R 52 -52 R 53 -26 R 79 0 R
52 26 R 53 52 R D 15001 17261 M 0 -368 R D 15001 17103 M 26 79 R 53 52 R
53 27 R 78 0 R D 16105 17366 M -52 52 R -79 27 R -105 0 R -79 -27 R
-53 -52 R 0 -53 R 27 -52 R 26 -27 R 52 -26 R 158 -53 R 53 -26 R 26 -26 R
26 -53 R 0 -79 R -52 -52 R -79 -26 R -105 0 R -79 26 R -53 52 R D
16394 17261 M -52 -27 R -53 -52 R -26 -79 R 0 -53 R 26 -79 R 53 -52 R
52 -26 R 79 0 R 53 26 R 53 52 R 26 79 R 0 53 R -26 79 R -53 52 R -53 27 R
-79 0 R D 16789 17445 M 0 -552 R D 16999 17261 M 0 -263 R 26 -79 R 53 -26 R
79 0 R 52 26 R 79 79 R D 17288 17261 M 0 -368 R D 17525 17445 M 0 -447 R
26 -79 R 53 -26 R 52 0 R D 17446 17261 M 184 0 R D 17788 17445 M 26 -27 R
26 27 R -26 26 R -26 -26 R D 17814 17261 M 0 -368 R D 18130 17261 M
-53 -27 R -53 -52 R -26 -79 R 0 -53 R 26 -79 R 53 -52 R 53 -26 R 78 0 R
53 26 R 53 52 R 26 79 R 0 53 R -26 79 R -53 52 R -53 27 R -78 0 R D
18524 17261 M 0 -368 R D 18524 17155 M 79 79 R 52 27 R 79 0 R 53 -27 R
26 -79 R 0 -262 R D 19444 17261 M 0 -263 R 26 -79 R 53 -26 R 79 0 R 52 26 R
79 79 R D 19733 17261 M 0 -368 R D 20128 17550 M -53 -53 R -53 -79 R
-52 -105 R -26 -131 R 0 -105 R 26 -132 R 52 -131 R 53 -79 R 53 -53 R D
20312 17261 M 0 -368 R D 20312 17103 M 26 79 R 52 52 R 53 27 R 79 0 R D
20706 16919 M -26 -26 R -27 26 R 27 26 R 26 -26 R 0 -79 R -26 -53 R
-27 -26 R D 20943 17445 M 0 -447 R 26 -79 R 52 -26 R 53 0 R D 20864 17261 M
184 0 R D 21205 17550 M 53 -53 R 53 -79 R 52 -105 R 27 -131 R 0 -105 R
-27 -132 R -52 -131 R -53 -79 R -53 -53 R D 40 setlinewidth 3996 2534 M
18935 0 R D 3996 2534 M 0 280 R D 20 setlinewidth 3954 2025 M -64 -21 R
-42 -63 R -21 -105 R 0 -63 R 21 -105 R 42 -63 R 64 -21 R 42 0 R 63 21 R
42 63 R 21 105 R 0 63 R -21 105 R -42 63 R -63 21 R -42 0 R D
40 setlinewidth 7783 2534 M 0 280 R D 20 setlinewidth 7678 1941 M 42 21 R
63 63 R 0 -441 R D 40 setlinewidth 11570 2534 M 0 280 R D 20 setlinewidth
11423 1920 M 0 21 R 21 42 R 21 21 R 42 21 R 84 0 R 42 -21 R 21 -21 R
21 -42 R 0 -42 R -21 -42 R -42 -63 R -211 -210 R 295 0 R D 40 setlinewidth
15357 2534 M 0 280 R D 20 setlinewidth 15231 2025 M 231 0 R -126 -168 R
63 0 R 42 -21 R 21 -21 R 21 -63 R 0 -42 R -21 -63 R -42 -42 R -63 -21 R
-63 0 R -63 21 R -21 21 R -21 42 R D 40 setlinewidth 19144 2534 M 0 280 R D
20 setlinewidth 19186 2025 M -210 -294 R 315 0 R D 19186 2025 M 0 -441 R D
40 setlinewidth 22931 2534 M 0 280 R D 20 setlinewidth 23015 2025 M -210 0 R
-21 -189 R 21 21 R 63 21 R 63 0 R 63 -21 R 42 -42 R 21 -63 R 0 -42 R
-21 -63 R -42 -42 R -63 -21 R -63 0 R -63 21 R -21 21 R -21 42 R D
40 setlinewidth 4374 2534 M 0 140 R D 4753 2534 M 0 140 R D 5132 2534 M
0 140 R D 5510 2534 M 0 140 R D 5889 2534 M 0 140 R D 6268 2534 M 0 140 R D
6647 2534 M 0 140 R D 7025 2534 M 0 140 R D 7404 2534 M 0 140 R D
8161 2534 M 0 140 R D 8540 2534 M 0 140 R D 8919 2534 M 0 140 R D
9298 2534 M 0 140 R D 9676 2534 M 0 140 R D 10055 2534 M 0 140 R D
10434 2534 M 0 140 R D 10812 2534 M 0 140 R D 11191 2534 M 0 140 R D
11948 2534 M 0 140 R D 12327 2534 M 0 140 R D 12706 2534 M 0 140 R D
13085 2534 M 0 140 R D 13463 2534 M 0 140 R D 13842 2534 M 0 140 R D
14221 2534 M 0 140 R D 14599 2534 M 0 140 R D 14978 2534 M 0 140 R D
15735 2534 M 0 140 R D 16114 2534 M 0 140 R D 16493 2534 M 0 140 R D
16872 2534 M 0 140 R D 17250 2534 M 0 140 R D 17629 2534 M 0 140 R D
18008 2534 M 0 140 R D 18386 2534 M 0 140 R D 18765 2534 M 0 140 R D
19523 2534 M 0 140 R D 19901 2534 M 0 140 R D 20280 2534 M 0 140 R D
20659 2534 M 0 140 R D 21037 2534 M 0 140 R D 21416 2534 M 0 140 R D
21795 2534 M 0 140 R D 22173 2534 M 0 140 R D 22552 2534 M 0 140 R D
20 setlinewidth 12222 1054 M 0 -294 R D 12222 928 M 21 63 R 42 42 R 43 21 R
63 0 R D 12727 1054 M 0 -294 R D 12727 991 M -42 42 R -42 21 R -63 0 R
-42 -21 R -42 -42 R -21 -63 R 0 -42 R 21 -63 R 42 -42 R 42 -21 R 63 0 R
42 21 R 42 42 R D 13127 1202 M 0 -442 R D 13127 991 M -42 42 R -42 21 R
-64 0 R -42 -21 R -42 -42 R -21 -63 R 0 -42 R 21 -63 R 42 -42 R 42 -21 R
64 0 R 42 21 R 42 42 R D 13274 1202 M 21 -21 R 21 21 R -21 21 R -21 -21 R D
13295 1054 M 0 -294 R D 13463 1054 M 0 -210 R 21 -63 R 42 -21 R 63 0 R
42 21 R 64 63 R D 13695 1054 M 0 -294 R D 14073 991 M -21 42 R -63 21 R
-63 0 R -63 -21 R -21 -42 R 21 -42 R 42 -21 R 105 -21 R 42 -21 R 21 -42 R
0 -21 R -21 -42 R -63 -21 R -63 0 R -63 21 R -21 42 R D 14557 1054 M
0 -294 R D 14557 928 M 21 63 R 42 42 R 42 21 R 63 0 R D 40 setlinewidth
3996 16512 M 18935 0 R D 3996 16512 M 0 -279 R D 7783 16512 M 0 -279 R D
11570 16512 M 0 -279 R D 15357 16512 M 0 -279 R D 19144 16512 M 0 -279 R D
22931 16512 M 0 -279 R D 4374 16512 M 0 -139 R D 4753 16512 M 0 -139 R D
5132 16512 M 0 -139 R D 5510 16512 M 0 -139 R D 5889 16512 M 0 -139 R D
6268 16512 M 0 -139 R D 6647 16512 M 0 -139 R D 7025 16512 M 0 -139 R D
7404 16512 M 0 -139 R D 8161 16512 M 0 -139 R D 8540 16512 M 0 -139 R D
8919 16512 M 0 -139 R D 9298 16512 M 0 -139 R D 9676 16512 M 0 -139 R D
10055 16512 M 0 -139 R D 10434 16512 M 0 -139 R D 10812 16512 M 0 -139 R D
11191 16512 M 0 -139 R D 11948 16512 M 0 -139 R D 12327 16512 M 0 -139 R D
12706 16512 M 0 -139 R D 13085 16512 M 0 -139 R D 13463 16512 M 0 -139 R D
13842 16512 M 0 -139 R D 14221 16512 M 0 -139 R D 14599 16512 M 0 -139 R D
14978 16512 M 0 -139 R D 15735 16512 M 0 -139 R D 16114 16512 M 0 -139 R D
16493 16512 M 0 -139 R D 16872 16512 M 0 -139 R D 17250 16512 M 0 -139 R D
17629 16512 M 0 -139 R D 18008 16512 M 0 -139 R D 18386 16512 M 0 -139 R D
18765 16512 M 0 -139 R D 19523 16512 M 0 -139 R D 19901 16512 M 0 -139 R D
20280 16512 M 0 -139 R D 20659 16512 M 0 -139 R D 21037 16512 M 0 -139 R D
21416 16512 M 0 -139 R D 21795 16512 M 0 -139 R D 22173 16512 M 0 -139 R D
22552 16512 M 0 -139 R D 3996 2534 M 0 13978 R D 3996 2534 M 378 0 R D
20 setlinewidth 2912 2976 M -63 -21 R -42 -63 R -21 -106 R 0 -63 R 21 -105 R
42 -63 R 63 -21 R 43 0 R 63 21 R 42 63 R 21 105 R 0 63 R -21 106 R -42 63 R
-63 21 R -43 0 R D 3249 2576 M -21 -21 R 21 -21 R 21 21 R -21 21 R D
3543 2976 M -63 -21 R -42 -63 R -21 -106 R 0 -63 R 21 -105 R 42 -63 R
63 -21 R 43 0 R 63 21 R 42 63 R 21 105 R 0 63 R -21 106 R -42 63 R -63 21 R
-43 0 R D 40 setlinewidth 3996 7193 M 378 0 R D 20 setlinewidth 2912 7382 M
-63 -21 R -42 -63 R -21 -106 R 0 -63 R 21 -105 R 42 -63 R 63 -21 R 43 0 R
63 21 R 42 63 R 21 105 R 0 63 R -21 106 R -42 63 R -63 21 R -43 0 R D
3249 6982 M -21 -21 R 21 -21 R 21 21 R -21 21 R D 3438 7277 M 0 21 R 21 42 R
21 21 R 42 21 R 85 0 R 42 -21 R 21 -21 R 21 -42 R 0 -42 R -21 -43 R
-42 -63 R -211 -210 R 295 0 R D 40 setlinewidth 3996 11853 M 378 0 R D
20 setlinewidth 2912 12041 M -63 -21 R -42 -63 R -21 -105 R 0 -63 R
21 -105 R 42 -63 R 63 -21 R 43 0 R 63 21 R 42 63 R 21 105 R 0 63 R -21 105 R
-42 63 R -63 21 R -43 0 R D 3249 11642 M -21 -21 R 21 -21 R 21 21 R -21 21 R
D 3628 12041 M -211 -294 R 316 0 R D 3628 12041 M 0 -441 R D 40 setlinewidth
3996 16512 M 378 0 R D 20 setlinewidth 2912 16511 M -63 -21 R -42 -64 R
-21 -105 R 0 -63 R 21 -105 R 42 -63 R 63 -21 R 43 0 R 63 21 R 42 63 R
21 105 R 0 63 R -21 105 R -42 64 R -63 21 R -43 0 R D 3249 16111 M -21 -21 R
21 -21 R 21 21 R -21 21 R D 3691 16447 M -21 43 R -63 21 R -43 0 R -63 -21 R
-42 -64 R -21 -105 R 0 -105 R 21 -84 R 42 -42 R 63 -21 R 22 0 R 63 21 R
42 42 R 21 63 R 0 21 R -21 63 R -42 42 R -63 21 R -22 0 R -63 -21 R
-42 -42 R -21 -63 R D 40 setlinewidth 3996 3699 M 189 0 R D 3996 4864 M
189 0 R D 3996 6029 M 189 0 R D 3996 8358 M 189 0 R D 3996 9523 M 189 0 R D
3996 10688 M 189 0 R D 3996 13018 M 189 0 R D 3996 14183 M 189 0 R D
3996 15348 M 189 0 R D 20 setlinewidth 1850 8724 M 211 0 R 63 21 R 21 42 R
0 63 R -21 42 R -63 63 R D 1850 8955 M 295 0 R D 1619 9271 M 42 -42 R
63 -42 R 84 -42 R 105 -21 R 85 0 R 105 21 R 105 42 R 63 42 R 42 42 R D
1850 9418 M 295 0 R D 1977 9418 M -64 21 R -42 42 R -21 42 R 0 63 R D
2124 9734 M 21 -22 R -21 -21 R -21 21 R 21 22 R 63 0 R 42 -22 R 21 -21 R D
1703 9923 M 358 0 R 63 21 R 21 42 R 0 42 R D 1850 9860 M 0 147 R D
1619 10133 M 42 42 R 63 42 R 84 42 R 105 21 R 85 0 R 105 -21 R 105 -42 R
63 -42 R 42 -42 R D 40 setlinewidth 22931 2534 M 0 13978 R D 22931 2534 M
-379 0 R D 22931 7193 M -379 0 R D 22931 11853 M -379 0 R D 22931 16512 M
-379 0 R D 22931 3699 M -190 0 R D 22931 4864 M -190 0 R D 22931 6029 M
-190 0 R D 22931 8358 M -190 0 R D 22931 9523 M -190 0 R D 22931 10688 M
-190 0 R D 22931 13018 M -190 0 R D 22931 14183 M -190 0 R D 22931 15348 M
-190 0 R D 4000 2586 M 665 7445 R 277 2149 R 213 1106 R 180 556 R 158 221 R
142 8 R 132 -129 R 122 -218 R 115 -271 R 109 -301 R 103 -315 R 99 -317 R
94 -313 R 92 -304 R 87 -291 R 85 -276 R 83 -262 R 80 -247 R 78 -232 R
76 -217 R 73 -205 R 73 -191 R 70 -180 R 69 -168 R 68 -159 R 66 -149 R
65 -140 R 64 -133 R 63 -125 R 61 -118 R 61 -112 R 60 -107 R 58 -101 R
58 -96 R 57 -92 R 56 -87 R 56 -84 R 54 -80 R 54 -76 R 54 -74 R 52 -70 R
52 -68 R 52 -65 R 50 -63 R 50 -61 R 50 -58 R 49 -57 R 49 -54 R 48 -53 R
47 -51 R 48 -49 R 46 -48 R 46 -47 R 46 -45 R 45 -44 R 45 -42 R 45 -41 R
44 -41 R 44 -39 R 43 -38 R 43 -37 R 43 -36 R 42 -36 R 42 -34 R 42 -34 R
41 -32 R 41 -32 R 41 -32 R 41 -30 R 40 -30 R 40 -29 R 39 -29 R 39 -28 R
40 -27 R 38 -27 R 39 -26 R 38 -26 R 38 -25 R 38 -25 R 37 -24 R 38 -24 R
37 -24 R 37 -22 R 36 -23 R 37 -22 R 36 -22 R 36 -21 R 36 -21 R 35 -20 R
36 -21 R 35 -20 R 35 -19 R 35 -19 R 34 -19 R 35 -19 R 34 -18 R 34 -18 R
34 -17 R 34 -18 R 33 -16 R D 20 setlinewidth 4964 14662 M 0 -298 R 17 -53 R
35 -17 R 36 0 R D 4911 14539 M 123 0 R D 5157 14504 M 315 0 R D 5157 14399 M
315 0 R D 5700 14662 M -53 -18 R -35 -52 R -17 -88 R 0 -53 R 17 -87 R
35 -53 R 53 -17 R 35 0 R 53 17 R 35 53 R 17 87 R 0 53 R -17 88 R -35 52 R
-53 18 R -35 0 R D 5980 14329 M -17 -18 R 17 -17 R 18 17 R -18 18 R D
6173 14592 M 35 17 R 53 53 R 0 -368 R D 6489 14574 M 0 18 R 17 35 R 18 17 R
35 18 R 70 0 R 35 -18 R 17 -17 R 18 -35 R 0 -35 R -18 -35 R -35 -53 R
-175 -175 R 246 0 R D 7032 14662 M -175 0 R -18 -158 R 18 18 R 52 17 R
53 0 R 52 -17 R 36 -35 R 17 -53 R 0 -35 R -17 -53 R -36 -35 R -52 -17 R
-53 0 R -52 17 R -18 18 R -17 35 R D 40 setlinewidth 4002 2571 M 940 5264 R
393 1520 R 300 782 R 254 393 R 224 156 R 202 6 R 186 -92 R 172 -153 R
163 -192 R 154 -213 R 146 -222 R 139 -225 R 134 -221 R 129 -215 R 124 -206 R
121 -195 R 116 -185 R 113 -175 R 110 -164 R 108 -154 R 104 -144 R 102 -135 R
100 -128 R 98 -119 R 95 -112 R 94 -105 R 92 -100 R 90 -93 R 89 -89 R
87 -83 R 86 -80 R 84 -75 R 83 -71 R 82 -68 R 81 -65 R 79 -62 R 79 -59 R
77 -57 R 76 -54 R 75 -52 R 75 -50 R 73 -48 R 73 -46 R 72 -44 R 71 -43 R
70 -41 R 69 -40 R 69 -39 R 68 -37 R 67 -36 R 67 -35 R 66 -34 R 65 -33 R
65 -32 R 64 -31 R 64 -30 R 63 -29 R 62 -28 R 62 -28 R 61 -27 R 61 -26 R
60 -26 R 60 -25 R 60 -24 R 59 -24 R 58 -23 R 58 -23 R 58 -22 R 57 -21 R
57 -22 R 56 -20 R 56 -21 R 56 -19 R 55 -20 R 55 -19 R 54 -18 R 54 -18 R
54 -18 R 54 -18 R 53 -17 R 52 -17 R 53 -16 R 52 -16 R 52 -16 R 51 -16 R
52 -15 R 50 -15 R 51 -15 R 50 -15 R 50 -14 R 50 -14 R 50 -14 R 49 -13 R
49 -14 R 48 -13 R 49 -13 R 48 -12 R 48 -13 R 48 -12 R 47 -12 R D
20 setlinewidth 5554 11217 M -52 -17 R -35 -53 R -18 -87 R 0 -53 R 18 -88 R
35 -52 R 52 -18 R 35 0 R 53 18 R 35 52 R 17 88 R 0 53 R -17 87 R -35 53 R
-53 17 R -35 0 R D 5835 10884 M -18 -17 R 18 -18 R 17 18 R -17 17 R D
5992 11130 M 0 17 R 18 35 R 17 18 R 35 17 R 71 0 R 35 -17 R 17 -18 R
18 -35 R 0 -35 R -18 -35 R -35 -52 R -175 -176 R 245 0 R D 6536 11217 M
-176 0 R -17 -157 R 17 17 R 53 18 R 53 0 R 52 -18 R 35 -35 R 18 -52 R
0 -35 R -18 -53 R -35 -35 R -52 -18 R -53 0 R -53 18 R -17 17 R -18 35 R D
40 setlinewidth 10690 5865 M 939 -392 R D 4004 2560 M 1331 3722 R 554 1075 R
426 553 R 358 278 R 317 111 R 285 4 R 263 -65 R 245 -109 R 229 -135 R
218 -151 R 206 -157 R 198 -159 R 189 -157 R 182 -151 R 176 -146 R 170 -138 R
165 -131 R 160 -123 R 156 -116 R 151 -109 R 148 -102 R 145 -96 R 141 -90 R
138 -84 R 135 -79 R 133 -75 R 130 -70 R 128 -66 R 125 -63 R 123 -59 R
121 -56 R 120 -53 R 117 -51 R 116 -48 R 114 -46 R 112 -44 R 111 -41 R
109 -40 R 108 -39 R 107 -36 R 105 -36 R 104 -34 R 103 -32 R 101 -32 R
100 -30 R 100 -29 R 98 -28 R 97 -28 R 96 -26 R 95 -25 R 94 -25 R 94 -24 R
92 -23 R 92 -23 R 90 -22 R 90 -21 R 89 -21 R 89 -20 R 87 -19 R 87 -19 R
86 -19 R 85 -18 R 85 -18 R 84 -17 R 83 -17 R 83 -16 R 82 -16 R 82 -16 R
81 -15 R 80 -15 R 80 -15 R 79 -14 R 78 -14 R 78 -14 R 78 -13 R 77 -13 R
77 -13 R 76 -13 R 75 -12 R 75 -12 R 75 -12 R 74 -12 R 74 -11 R 73 -11 R
73 -12 R 72 -10 R 72 -11 R 72 -10 R 71 -11 R 71 -10 R 70 -10 R 70 -10 R
70 -9 R 69 -10 R 69 -9 R 68 -9 R 68 -9 R 68 -9 R 68 -8 R 67 -9 R D
20 setlinewidth 6830 8782 M -52 -18 R -35 -52 R -18 -88 R 0 -52 R 18 -88 R
35 -53 R 52 -17 R 35 0 R 53 17 R 35 53 R 18 88 R 0 52 R -18 88 R -35 52 R
-53 18 R -35 0 R D 7111 8449 M -18 -18 R 18 -17 R 17 17 R -17 18 R D
7461 8782 M -175 0 R -17 -158 R 17 18 R 53 17 R 52 0 R 53 -17 R 35 -35 R
17 -53 R 0 -35 R -17 -53 R -35 -35 R -53 -17 R -52 0 R -53 17 R -17 18 R
-18 35 R D 40 setlinewidth 13463 4889 M 1972 -398 R D 4008 2552 M
1881 2633 R 784 759 R 602 391 R 508 197 R 447 78 R 404 3 R 371 -46 R
346 -77 R 325 -95 R 307 -107 R 293 -111 R 279 -113 R 268 -110 R 258 -107 R
248 -103 R 241 -98 R 233 -93 R 226 -87 R 220 -82 R 215 -77 R 209 -72 R
204 -68 R 200 -63 R 195 -60 R 191 -56 R 188 -53 R 184 -49 R 180 -47 R
178 -44 R 174 -42 R 171 -40 R 169 -37 R 166 -36 R 164 -34 R 161 -33 R
159 -31 R 156 -29 R 155 -28 R 153 -27 R 150 -26 R 149 -25 R 147 -24 R
145 -23 R 144 -23 R 142 -21 R 140 -21 R 139 -20 R 137 -19 R 136 -19 R
135 -18 R 133 -17 R 132 -17 R 131 -16 R 129 -16 R 128 -16 R 127 -15 R
126 -14 R 125 -15 R 124 -14 R 123 -13 R 121 -13 R 121 -13 R 120 -12 R
119 -13 R 118 -11 R 117 -12 R 116 -11 R 115 -11 R 114 -11 R 114 -11 R
113 -10 R 112 -10 R 111 -10 R 110 -10 R 110 -9 R 109 -10 R 108 -9 R 108 -9 R
107 -8 R 106 -9 R 105 -8 R 105 -9 R 104 -8 R 104 -8 R 103 -7 R 102 -8 R
102 -8 R 101 -7 R 101 -7 R 100 -8 R 100 -7 R 99 -6 R 98 -7 R 98 -7 R 97 -6 R
97 -7 R 97 -6 R 96 -6 R 95 -6 R 95 -6 R D 20 setlinewidth 8317 6990 M
35 17 R 53 53 R 0 -368 R D 40 setlinewidth 17385 4199 M 1994 -207 R D
4013 2547 M 2660 1861 R 1110 538 R 851 276 R 717 139 R 632 55 R 572 2 R
526 -32 R 489 -54 R 459 -68 R 435 -75 R 413 -79 R 395 -80 R 379 -78 R
364 -76 R 352 -72 R 340 -70 R 330 -65 R 320 -62 R 311 -58 R 303 -54 R
296 -51 R 289 -48 R 282 -45 R 276 -42 R 271 -40 R 265 -37 R 260 -35 R
255 -33 R 251 -31 R 247 -30 R 242 -28 R 239 -27 R 235 -25 R 231 -24 R
228 -23 R 225 -22 R 221 -21 R 219 -20 R 216 -19 R 213 -18 R 210 -18 R
208 -17 R 205 -16 R 203 -16 R 201 -15 R 199 -15 R 196 -14 R 194 -13 R
193 -13 R 190 -13 R D 20 setlinewidth 10036 5754 M 0 18 R 18 35 R 17 17 R
35 18 R 70 0 R 35 -18 R 18 -17 R 17 -35 R 0 -35 R -17 -35 R -35 -53 R
-175 -175 R 245 0 R D 40 setlinewidth 22931 3712 M Z 4020 2543 M 3763 1316 R
1568 380 R 1204 196 R 1015 98 R 894 39 R 808 2 R 743 -23 R 692 -39 R
650 -48 R 614 -53 R 585 -56 R 558 -56 R 536 -55 R 515 -54 R 498 -51 R
481 -49 R 466 -46 R 453 -44 R 440 -41 R 429 -38 R 418 -37 R 408 -33 R
400 -32 R 390 -30 R 383 -28 R D 20 setlinewidth 12674 4981 M -175 -245 R
263 0 R D 12674 4981 M 0 -368 R D 40 setlinewidth 12895 7193 M 8142 0 R
0 8155 R -8142 0 R 0 -8155 R D 16966 12901 M 29 0 R 28 -1 R 28 -1 R 29 -2 R
28 -2 R 28 -3 R 29 -3 R 28 -4 R 28 -4 R 28 -4 R 28 -6 R 28 -5 R 28 -6 R
27 -7 R 28 -7 R 27 -8 R 27 -8 R 27 -9 R 27 -9 R 27 -9 R 27 -10 R 26 -10 R
27 -11 R 26 -12 R 25 -11 R 26 -13 R 26 -12 R 25 -14 R 25 -13 R 24 -14 R
25 -15 R 24 -15 R 24 -15 R 24 -16 R 23 -16 R 23 -16 R 23 -17 R 23 -17 R
22 -18 R 22 -18 R 22 -19 R 21 -19 R 21 -19 R 20 -19 R 21 -20 R 20 -21 R
19 -20 R 19 -21 R 19 -22 R 19 -21 R 18 -22 R 17 -22 R 18 -23 R 17 -23 R
16 -23 R 16 -24 R 16 -23 R 15 -24 R 15 -25 R 14 -24 R 14 -25 R 14 -25 R
13 -25 R 13 -26 R 12 -25 R 12 -26 R 11 -26 R 11 -27 R 11 -26 R 9 -27 R
10 -27 R 9 -27 R 9 -27 R 8 -27 R 7 -27 R 7 -28 R 7 -28 R 6 -27 R 6 -28 R
5 -28 R 5 -28 R 4 -29 R 4 -28 R 3 -28 R 2 -28 R 3 -29 R 1 -28 R 2 -29 R
0 -28 R 1 -29 R -1 -28 R 0 -28 R -2 -29 R -1 -28 R -3 -29 R -2 -28 R
-3 -28 R -4 -28 R -4 -29 R -5 -28 R -5 -28 R -6 -28 R -6 -27 R -7 -28 R
-7 -28 R -7 -27 R -8 -27 R -9 -27 R -9 -27 R -10 -27 R -9 -27 R -11 -26 R
-11 -27 R -11 -26 R -12 -26 R -12 -25 R -13 -26 R -13 -25 R -14 -25 R
-14 -25 R -14 -24 R -15 -25 R -15 -24 R -16 -23 R -16 -24 R -16 -23 R
-17 -23 R -18 -23 R -17 -22 R -18 -22 R -19 -21 R -19 -22 R -19 -21 R
-19 -20 R -20 -21 R -21 -20 R -20 -19 R -21 -19 R -21 -19 R -22 -19 R
-22 -18 R -22 -18 R -23 -17 R -23 -17 R -23 -16 R -23 -17 R -24 -15 R
-24 -16 R -24 -14 R -25 -15 R -24 -14 R -25 -13 R -25 -14 R -26 -12 R
-26 -13 R -25 -11 R -26 -12 R -27 -11 R -26 -10 R -27 -10 R -27 -9 R
-27 -10 R -27 -8 R -27 -8 R -27 -8 R -28 -7 R -27 -7 R -28 -6 R -28 -5 R
-28 -6 R -28 -4 R -28 -4 R -28 -4 R -29 -3 R -28 -3 R -28 -2 R -29 -2 R
-28 -1 R -28 -1 R -29 0 R -28 0 R -29 1 R -28 1 R -28 2 R -29 2 R -28 3 R
-28 3 R -28 4 R -29 4 R -28 4 R -27 6 R -28 5 R -28 6 R -28 7 R -27 7 R
-28 8 R -27 8 R -27 8 R -27 10 R -27 9 R -26 10 R -27 10 R -26 11 R -26 12 R
-26 11 R -26 13 R -25 12 R -25 14 R -25 13 R -25 14 R -24 15 R -25 14 R
-24 16 R -23 15 R -24 17 R -23 16 R -23 17 R -22 17 R -23 18 R -21 18 R
-22 19 R -21 19 R -21 19 R -21 19 R -20 20 R -20 21 R -20 20 R -19 21 R
-19 22 R -18 21 R -18 22 R -18 22 R -17 23 R -17 23 R -17 23 R -16 24 R
-15 23 R -16 24 R -15 25 R -14 24 R -14 25 R -14 25 R -13 25 R -12 26 R
-13 25 R -11 26 R -12 26 R -11 27 R -10 26 R -10 27 R -9 27 R -9 27 R
-9 27 R -8 27 R -8 27 R -7 28 R -6 28 R -7 27 R -5 28 R -5 28 R -5 28 R
-4 29 R -4 28 R -3 28 R -3 28 R -2 29 R -2 28 R -1 29 R -1 28 R 0 28 R
0 29 R 1 28 R 1 29 R 2 28 R 2 29 R 3 28 R 3 28 R 4 28 R 4 29 R 5 28 R 5 28 R
5 28 R 7 27 R 6 28 R 7 28 R 8 27 R 8 27 R 9 27 R 9 27 R 9 27 R 10 27 R
10 26 R 11 27 R 12 26 R 11 26 R 13 25 R 12 26 R 13 25 R 14 25 R 14 25 R
14 24 R 15 25 R 16 24 R 15 23 R 16 24 R 17 23 R 17 23 R 17 23 R 18 22 R
18 22 R 18 21 R 19 22 R 19 21 R 20 20 R 20 21 R 20 20 R 21 19 R 21 19 R
21 19 R 22 19 R 21 18 R 23 18 R 22 17 R 23 17 R 23 16 R 24 16 R 23 16 R
24 15 R 25 15 R 24 15 R 25 14 R 25 13 R 25 14 R 25 12 R 26 13 R 26 11 R
26 12 R 26 11 R 27 10 R 26 10 R 27 9 R 27 9 R 27 9 R 27 8 R 28 8 R 27 7 R
28 7 R 28 6 R 28 5 R 27 6 R 28 4 R 29 4 R 28 4 R 28 3 R 28 3 R 29 2 R 28 2 R
28 1 R 29 1 R 28 0 R 0 1631 R 377 -653 R D 16966 14532 M -377 -653 R D
18118 12424 M 1151 1153 R -194 -729 R D 19269 13577 M -728 -196 R D
18595 11270 M 1628 0 R -653 -377 R D 20223 11270 M -653 378 R D
18118 10117 M 1151 -1153 R -728 196 R D 19269 8964 M -194 729 R D
16966 9640 M 0 -1631 R -377 653 R D 16966 8009 M 377 653 R D 15815 10117 M
-1152 -1153 R 195 729 R D 14663 8964 M 729 196 R D 15338 11270 M -1629 0 R
653 378 R D 13709 11270 M 653 -377 R D 15815 12424 M -1152 1153 R 729 -196 R
D 14663 13577 M 195 -729 R D
%%PageTrailer
showpage
end restore
%%PageResources: font Helvetica
%%Trailer
restore
%%Pages: 1
%%DocumentNeededResources: font Helvetica
%%EOF

